Convexification numerical algorithm for a 2D inverse scattering problem with backscatter data

This paper is concerned with the inverse scattering problem which aims to determine the spatially distributed dielectric constant coefficient of the 2D Helmholtz equation from multifrequency backscatter data associated with a single direction of the incident plane wave. We propose a globally convergent convexification numerical algorithm to solve this nonlinear and ill-posed inverse problem. The key advantage of our method over conventional optimization approaches is that it does not require a good first guess about the solution. First, we eliminate the coefficient from the Helmholtz equation using a change of variables. Next, using a truncated expansion with respect to a special Fourier basis, we approximately reformulate the inverse problem as a system of quasilinear elliptic PDEs, which can be numerically solved by a weighted quasi-reversibility approach. The cost functional for the weighted quasi-reversibility method is constructed as a Tikhonov-like functional that involves a Carleman Weight Function. Our numerical study shows that, using a version of the gradient descent method, one can find the minimizer of this Tikhonov-like functional without any advanced \emph{a priori} knowledge about it.

==> mathmacros.tex <==
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\renewcommand{\phi}{\varphi}
\renewcommand{\d}{\mathrm{d}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\ol}{\overline}
\renewcommand{\i}{\mathrm{i}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\mur}{\mu_{\mathrm{r}}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\per}{\mathrm{per}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\smooth}{\text{sm}}
\newcommand{\RR}{R}
\newcommand{\T}{\mathcal{T}}
\renewcommand{\sc}{\mathrm{sc}}
\newcommand{\inc}{\mathrm{inc}}


\DeclareMathOperator{\sign}{\mathrm{sign}}
\DeclareMathOperator{\Id}{\mathrm{Id}}


 \newtheorem{remark}[theorem]{Remark}

\renewcommand{\Re}{\mathrm{Re}\,}
\renewcommand{\Im}{\mathrm{Im}\,}
 \newcommand{\smalf}{\par\smallskip\noindent}
 \newcommand{\medlf}{\par\medskip\noindent}
 \newcommand{\biglf}{\par\bigskip\noindent}

\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsi}{\epsilon}
\newcommand{\oD}{\overline{D}}
\newcommand{\oS}{\overline{S}}
\newcommand{\ov}{\overline}
\newcommand{\pD}{\partial D}
\newcommand{\cO}{{\cal O}}
\newcommand{\bH}{{\bm{H}}}
\newcommand{\vbH}{{\vec{\bm{H}}}}
\newcommand{\bE}{{\bm{E}}}
\newcommand{\vbE}{{\vec{\bm{E}}}}
\newcommand{\vbJ}{{\vec{\bf J}}}
\newcommand{\vbA}{\mathcal{\bm{A}}}
\newcommand{\bD}{{\bm{D}}}
\newcommand{\bRe}{{\bm{\mathcal{R}}^\epsilon}}
\newcommand{\bTe}{{\bm{\mathcal{T}}^\epsilon}}
\newcommand{\vbD}{{\vec{\bm{D}}}}
\newcommand{\curl}{{\vec{\nabla}\times}}
\newcommand{\divv}{{\vec{\nabla}\cdot}}
\renewcommand{\div}{\mathrm{div}}
\newcommand{\curll}{\mathrm{curl}}
\newcommand{\divtt}{{\nabla^\bot\cdot}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cR}{{\cal R}}
\newcommand{\pa}{\partial}
\newcommand{\nal}{\nabla_{\alpha}}
\newcommand{\nalT}{\nabla_{\alpha,T}}
\newcommand{\naT}{\nabla_T}
\newcommand{\intO}{\int_{\Omega}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
%\newcommand{\vbz}{\vec{\bm{z}}}
%\newcommand{\vx}{\vbx}
%\newcommand{\bx}{\bm{x}}
%\newcommand{\vbn}{\vec{\bm{n}}}
%\newcommand{\vbut}{\vec{\bm{u}}^t}
%\newcommand{\vbui}{\vec{\bm{u}}^i}
%\newcommand{\vbuis}{\vec{\bm{u}}^{i(s')}}
%\newcommand{\vbu}{\vec{\bm{u}}}
%\newcommand{\vbg}{\vec{\bm{g}}}
%\newcommand{\vbf}{\vec{\bm{f}}}
%\newcommand{\vbw}{\vec{\bm{w}}}
%\newcommand{\vbv}{\vec{\bm{v}}}
%\newcommand{\vbphi}{\vec{\bm{\varphi}}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cm}{{\mathcal M}}
\newcommand{\lin}{\big<}
\newcommand{\rin}{\big>}
\newcommand{\bV}{\boldsymbol{\mathcal{V}}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bd}{{\bf d}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\icu}{{\mbox{\tiny curl}}}
\newcommand{\idiv}{{\mbox{\tiny div}}}

